Exploring deep learning for Event-Based Saliency Prediction with a Transformer-based model

Saliency prediction has been extensively studied in RGB images and videos as a computational model of human visual attention. In contrast, predicting saliency from event-based data remains largely unexplored, despite the biological inspiration and favorable sensing properties of event cameras. Two obstacles have held this direction back: the absence of large-scale event saliency datasets, and the lack of a strong baseline. In this paper, we introduce SEST (Swin Event-based Saliency Transformer), a transformer-based model for saliency prediction from event data, bridging the data scarcity barrier through event-native pretraining and synthetic supervision. SEST leverages a self-supervised pretrained event-based Swin Transformer backbone combined with a lightweight CNN decoder to produce dynamic saliency maps. To address the scarcity of annotated event-based saliency data, we introduce two new benchmark datasets, N-DHF1K and N-UCF Sports, generated from large-scale RGB saliency benchmarks. Experimental results show that SEST clearly outperforms existing event-based saliency methods and narrows the performance gap with state-of-the-art RGB models. Zero-shot evaluation on a real event camera dataset further demonstrates that our model trained on synthetic data remains transferable on real event streams. To the best of our knowledge, this work is the first to apply deep learning to event-based saliency prediction, opening a new research direction at the intersection of event-based vision and neuromorphic visual attention.

==> sec/3_Results___Disc.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%% EXPERIMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:exps}
%%%%%%%%%%%%%%%%%%%%%%%%%%% DATASETS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Saliency datasets}

 We converted two existing video saliency datasets (DHF1K \cite{wangRevisitingVideoSaliency2018}, and UCF Sports \cite{mathe2014actions}) into event datasets (N-DHF1K and N-UCF Sports) using ESIM library\cite{Gehrig_2020_CVPR} with positive and negative contrast thresholds of 0.09 and a 3 ms refractory period. We used their saliency and fixation maps as ground truths to train our model on the synthetic events.

\subsubsection{DHF1K}
Dynamic Human Fixations 1K (DHF1K) is a large-scale dataset of gaze recordings from 17 observers who were asked to freely view the videos. It consists of 1K videos with diverse content, varied motion and various objects. The original dataset was partitioned into 600 training, 100 validation, and 300 test videos. Since the ground truth labels for the official test are hidden for benchmarking, we reserved 100 videos from the training set to serve our test set. This resulted in a final split of 500 training videos, 100 validation videos, and 100 test videos.
\subsubsection{UCF Sports}
UCF Sports is a human fixations dataset on 150 videos from the UCF Sports Action dataset. The videos covered 9 action sports such as swinging, diving, and lifting. Contrary to DHF1K, where observers freely observed the videos, observers were asked to identify occurring actions within the UCF videos. Our final data split consists of 103 training videos, 15 validation videos, and a test set of 32 videos.

Although the proposed datasets are synthetically generated from RGB videos, this approach enables scalable supervision using high-quality human fixation data that is currently unavailable in native event-based form. More importantly, prior work has shown that event representations generated from photorealistic videos preserve motion, contrast, and temporal saliency cues relevant to downstream tasks \cite{Gehrig_2020_CVPR, yang2024event}. 
%Our results demonstrate consistent performance gains across two distinct datasets, suggesting that the learned representations capture generalizable saliency patterns rather than dataset-specific artifacts.

% \subsection{Saliency metrics}
% \noindent For a comprehensive analysis, we have used 5 different metrics, since each metric measures different properties of the heatmaps. 

% \subsubsection{AUC-Judd}
% The Area Under the ROC Curve (AUC) using the Judd method evaluates the agreement between a predicted saliency map $S$ and a set of human fixation points $F$. Each pixel in $S$ is treated as a binary classifier for fixation presence. By varying a threshold over $S$ and computing the true positive rate (TPR) and false positive rate (FPR) with respect to $F$, the ROC curve is obtained.

% \subsubsection{Normalized scanpath saliency }
% NSS measures the correspondence between a predicted saliency map $S$ and human fixation locations by first normalizing $S$ to zero mean and unit standard deviation, and then averaging the normalized values at fixation points:
% \begin{equation}
% \text{NSS} = \frac{1}{N} \sum_{i=1}^{N} \hat{S}(x_i, y_i), \quad 
% \hat{S} = \frac{S - \mu_S}{\sigma_S}
% \end{equation}
% where $(x_i, y_i)$ are the $N$ human fixation points, and $\mu_S$ and $\sigma_S$ denote the mean and standard deviation of $S$. Higher NSS values indicate that predicted saliency aligns more strongly with actual human fixations.

% \subsubsection{Similarity }
% \noindent The \textit{similarity (SIM)} metric \cite{swain1991color} measures the degree of overlap between two heatmaps \( X \) and \( Y \) by summing the minimum value at each corresponding pixel position (Eq.~\ref{eq:SIM}). Both maps are normalized such that the sum of all pixel values equals 1 to ensure that SIM ranges between 0 and 1 (1 indicates a perfect match and 0 means no similarity between heatmaps).
% \begin{equation}
% \text{SIM}(X, Y) = \sum_{i} \min(X_i, Y_i)
% \label{eq:SIM}
% \end{equation}


\subsection{Protocol}
\subsubsection{Implementation details}
SEST is implemented using the PyTorch framework. We use a batch size of 20 and a learning rate of 0.006. We train our model on a single NVIDIA H100 GPU on a server for 30 epochs with an AdamW optimizer \cite{loshchilovdecoupled}. We implement early stopping based on the validation loss (patience = 3) and reduce the learning rate on plateau by a factor of 0.1 (patience = 1). We trained and evaluated our model using various temporal window sizes by varying the number of bins ($T \in \{7, 10, 14, 21\}$) across the two datasets. The duration of each bin was fixed to match the sampling period of the original source videos. For N-UCF Sports (10Hz), the bin duration was set to 100ms, while for N-DHF1K (30Hz), it was set to 33.33ms. Consequently, the total observation window for each experiment scales linearly with the number of bins.

\subsubsection{Loss function}
We considered different metrics to design our loss function, following common practice in the literature \cite{bylinskiiWhatDifferentEvaluation2019}. Let $Y$ denote the ground truth saliency map and $\hat{Y}$ the predicted saliency map. The loss function is defined as: 
\begin{equation}
\mathcal{L}(\hat{Y}, Y)= \mathcal{L}_{\mathrm{KL}}(\hat{Y}, Y) + \alpha_1\mathcal{L}_{\mathrm{CC}}(\hat{Y}, Y) + \alpha_2\mathcal{L}_{\mathrm{BCE}}(\hat{Y}, Y)
\end{equation}
 with $\alpha_1 = 0.5$ and $\alpha_2 = 0.7$ set empirically. $ \mathcal{L}_{\mathrm{KL}}$, $\mathcal{L}_{\mathrm{CC}}$ and $\mathcal{L}_{\mathrm{BCE}}$ are \textit{Kullback-Leibler divergence}, \textit{Pearson Correlation Coefficient}, and \textit{Binary Cross Entropy} respectively. $ \mathcal{L}_{\mathrm{KL}} $ and $\mathcal{L}_{\mathrm{CC}}$ supervise the predicted saliency at the distribution level, while $\mathcal{L}_{\mathrm{BCE}}$ enforces pixel-wise localization, balancing distribution-matching with spatial accuracy. We negate the Pearson correlation so that minimizing $\mathcal{L}_{\mathrm{CC}}$ maximizes the correlation between $Y$ and $\hat{Y}$.

$ \mathcal{L}_{\mathrm{KL}} $ implements the \textit{Kullback-Leibler Divergence}, which quantifies the dissimilarity between two probability distributions:\\
\begin{equation}
\mathcal{L}_{\mathrm{KL}}(\hat{Y}, Y) = \sum_{x} {Y(x)} \log( \frac{Y(x)}{\hat{Y}(x)})
\end{equation} 


$\mathcal{L}_{\mathrm{CC}}$ implements the \textit{Pearson Correlation Coefficient} that measures the linear relationship between two images:

\begin{equation}
\mathcal{L}_{\mathrm{CC}}(\hat{Y},Y) = - \frac{\sum_{i} (\hat{Y}_i - \bar{\hat{Y}})(Y_i - \bar{Y})}{\sqrt{\sum_{i} (\hat{Y}_i - \bar{\hat{Y}})^2} \sqrt{\sum_{i} (Y_i - \bar{Y})^2}}
\end{equation} 

\subsubsection{Evaluation metrics}
We evaluate our model performance by employing the following metrics: AUC-Judd (AUC-J), Pearson Correlation Coefficient (CC), Similarity (SIM), and Normalized Scanpath Saliency (NSS). These metrics have been discussed in detail in \cite{bylinskiiWhatDifferentEvaluation2019}. 

\section{Results and Analysis}
\label{sec:res_analys}
\subsection{Performance results}
We compared the saliency prediction performance of our event-based model, SEST, on the N-DHF1K and N-UCF Sports datasets to the performance of two state-of-the-art event-based models (SNNevProto \cite{dangeloEventDrivenBioinspired2022} and evST \cite{chane2024event}) and several state-of-art RGB-based models from DHF1K and UCF Sports benchmarks\footnote{\href{https://mmcheng.net/videosal}{https://mmcheng.net/videosal}} (see Table \ref{tab:comparison}). 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.82\textwidth]{figs/vizualization_final.png}
    \caption{Illustration of qualitative results for three samples: UCF Sports Run-side-004 (rows 1-2), DHF1K  548 (rows 3-4), UCF Sports Swing-Bench-003 (rows 5-6).}
    \label{fig:viz}
\end{figure*}


\subsubsection{N-DHF1K} The best overall performance on this dataset is achieved by RGB-based models, with SalFoM leading across all four metrics. Other RGB-based models such as TMFI, THTD-Net, and STSANet follow closely. In contrast, existing event-based models show significantly inferior performance, with very low CC and NSS values. Our model, SEST, substantially improves performance within the event domain. Across different time bin configurations, SEST achieves AUC-J values up to 0.9197, CC up to 0.4907, SIM up to 0.3969, and NSS up to 2.3956, clearly outperforming all other event-based approaches by a large margin. 

\subsubsection{N-UCF Sports} Similar to the case of DHF1K, RGB models achieve the highest overall performance on this dataset too. Among them, the best performance is generally achieved by STSANet and TMFI, with AUC-J values of 0.936 and strong NSS scores. In comparison, existing event-based models exhibit noticeably lower performance, with AUC-J values typically in the range of 0.77 to 0.81 and NSS scores mostly below 1.5, highlighting the gap that remains between RGB-based methods and current event-based methods. However, SEST consistently outperforms all other event-based models across all four metrics. In particular, our model attains the highest AUC-J value among the event-based approaches, along with improved CC, SIM and NSS scores. Notably, the 14-bin configuration of our model provides the best overall performance. 

These results show that although a performance gap still exists between RGB and event-based methods, SEST significantly narrows this gap and sets a new state of the art for event-based saliency prediction on the DHF1K and UCF Sports datasets.  


\begin{table*}[!hbt]
    \centering
    \caption{Quantitative comparison on N-DHF1K and N-UCF Sports datasets.}
    \label{tab:comparison}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{5pt}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{llccccc|llccccc}
            \toprule
            \multicolumn{7}{c|}{\textbf{N-DHF1K}} & \multicolumn{7}{c}{\textbf{N-UCF Sports}} \\
            \midrule
            \textbf{Domain} & \textbf{Model} & \textbf{\#bins} & \textbf{AUC-J}$\uparrow$ & \textbf{CC}$\uparrow$ & \textbf{SIM}$\uparrow$ & \textbf{NSS}$\uparrow$ &
            \textbf{Domain} & \textbf{Model} & \textbf{\#bins} & \textbf{AUC-J}$\uparrow$ & \textbf{CC}$\uparrow$ & \textbf{SIM}$\uparrow$ & \textbf{NSS}$\uparrow$ \\
            \midrule
            \multirow{5}{*}{RGB}
            & \textbf{SalFoM}~\cite{moradi2024salfom}        & - & \textbf{0.9222} & \textbf{0.5692} & \textbf{0.4208} & \textbf{3.3536} &
            \multirow{5}{*}{RGB}
            & \textbf{TMFI}~\cite{10130326zhou}              & - & \textbf{0.936} & \textbf{0.707} & \textbf{0.565} & 3.863 \\
            & \textbf{TMFI}~\cite{10130326zhou}              & - & 0.9153 & 0.5461 & 0.4068 & 3.1463 &
            & \textbf{STSANet}~\cite{Wang_2023}              & - & \textbf{0.936} & 0.705 & 0.560 & \textbf{3.908} \\
            & \textbf{THTD-Net}~\cite{Moradi2024}            & - & 0.9152 & 0.5479 & 0.4062 & 3.1385 &
            & \textbf{SalSAC}~\cite{wu2020salsac}            & - & 0.926 & 0.671 & 0.534 & 3.523 \\
            & \textbf{STSANet}~\cite{Wang_2023}              & - & 0.9125 & 0.5288 & 0.3829 & 3.0103 &
            & \textbf{ViNet}~\cite{jain2021vinet}            & - & 0.924 & 0.673 & 0.522 & 3.620 \\
            & \textbf{TSFP-Net}~\cite{chang2021temporalspatialfeaturepyramidvideo} & - & 0.9116 & 0.5168 & 0.3921 & 2.9665 &
            & \textbf{TSFP-Net}~\cite{chang2021temporalspatialfeaturepyramidvideo} & - & 0.923 & 0.685 & 0.561 & 3.698 \\
            \midrule
            \multirow{9}{*}{Event}
            & \textbf{evST}~\cite{chane2024event}            & 21 & 0.5464 & 0.0274 & 0.1106 & 0.1420 &
            \multirow{9}{*}{Event}
            & \textbf{evST}~\cite{chane2024event}            & 21 & 0.7756 & 0.2681 & 0.1464 & 1.3312 \\
            & \textbf{evST}~\cite{chane2024event}            & 14 & 0.5408 & 0.0232 & 0.1208 & 0.1091 &
            & \textbf{evST}~\cite{chane2024event}            & 14 & 0.7779 & 0.2658 & 0.1382 & 1.3692 \\
            & \textbf{evST}~\cite{chane2024event}            & 10 & 0.5413 & 0.0246 & 0.1290 & 0.1120 &
            & \textbf{evST}~\cite{chane2024event}            & 10 & 0.7793 & 0.2594 & 0.1308 & 1.3798 \\
            & \textbf{evST}~\cite{chane2024event}            &  7 & 0.5380 & 0.0217 & 0.1317 & 0.0898 &
            & \textbf{evST}~\cite{chane2024event}            &  7 & 0.7787 & 0.2559 & 0.1263 & 1.3798 \\
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 21 & 0.6427 & 0.0753 & 0.1092 & 0.3999 &
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 21 & 0.7890 & 0.2325 & 0.1336 & 1.0205 \\
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 14 & 0.6201 & 0.0579 & 0.1185 & 0.2886 &
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 14 & 0.8195 & 0.2741 & 0.1369 & 1.2204 \\
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 10 & 0.6036 & 0.0443 & 0.1266 & 0.2054 &
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 10 & 0.7941 & 0.2237 & 0.1144 & 1.0474 \\
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} &  7 & 0.5884 & 0.0375 & 0.1342 & 0.1725 &
            & \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} &  7 & 0.8316 & 0.2834 & 0.1262 & 1.3286 \\
            & \textbf{SEST (this work)}                                  & 21 & 0.8956 & 0.4284 & 0.3014 & 2.1209 &
            & \textbf{SEST (this work)}                                  & 21 & 0.8605 & 0.4381 & 0.3090 & 2.1259 \\
            & \textbf{SEST (this work)}                                  & 14 & 0.9009 & 0.4814 & 0.3641 & 2.2769 &
            & \textbf{SEST (this work)}                                  & 14 & \textbf{0.8943} & \textbf{0.5237} & \textbf{0.3800} & \textbf{2.6590} \\
            & \textbf{SEST (this work)}                                  & 10 & 0.8947 & \textbf{0.4907} & \textbf{0.3969} & 2.2328 &
            & \textbf{SEST (this work)}                                  & 10 & 0.8942 & 0.5073 & 0.3462 & 2.6022 \\
            & \textbf{SEST (this work)}                      &  7 & \textbf{0.9197} & 0.4661 & 0.3634 & \textbf{2.3956} &
            & \textbf{SEST (this work)}                      &  7 & 0.8841 & 0.4555 & 0.3214 & 2.4537 \\
            \bottomrule
        \end{tabular}
    }
\end{table*}


\subsubsection{Qualitative analysis}
Figure~\ref{fig:viz} presents qualitative comparisons across three representative sequences: a high-motion athletics scene, a low-motion pedestrian scene, and a gymnastics scene. In all three cases, SEST produces spatially coherent, temporally consistent saliency maps that closely match the ground truth. SNNevProto generates diffuse activations dominated by background structure, failing to isolate salient subjects, while evST produces noisy, unstructured responses that deteriorate further in low-activity scenes. These observations highlight two consistent advantages of SEST over prior methods: robustness to varying event density, and temporal consistency across bins, both essential properties for reliable event-based saliency prediction in practice.

%\subsubsection{Evaluation on a real event dataset}
%To assess the generalization capability of SEST beyond synthetic data, we conduct a zero-shot evaluation on the real event camera dataset of Chane~et~al.~\cite{chane2024event} using 14 temporal bins. No fine-tuning is performed. As reported in Table~\ref{tab:real}, SEST achieves an AUC-J of 0.7725, CC of 0.4725, SIM of 0.4708, and NSS of 1.1434, remaining competitive with its synthetic performance on N-DHF1K at the same bin configuration. SNNevProto fails to generalise, scoring substantially lower across all metrics. evST obtains a higher NSS (1.4141) but lower CC and SIM (0.2750 and 0.1396) --- a result likely attributable to the predominantly low-to-medium motion activity in the real dataset, which favours simpler event-based models less exposed  to high-motion scenes. This highlights a key limitation of current real event saliency benchmarks and further motivates the utility of N-DHF1K and N-UCF Sports, which cover a broader and more challenging range of motion dynamics, as essential resources for training future robust event-based saliency models.

%\begin{table}[hbt!]
%    \centering
%    \caption{Zero-shot evaluation on the real event camera dataset 
%    of Chane~et~al.~\cite{chane2024event} (14 bins). No fine-tuning 
%    is performed.}
%    \label{tab:real}
%   \renewcommand{\arraystretch}{1.2}
%    \setlength{\tabcolsep}{6pt}
%    \resizebox{0.48\textwidth}{!}{
%        \begin{tabular}{lcccc}
%            \toprule
%            \textbf{Model} & \textbf{AUC-J}$\uparrow$ & \textbf{CC}$\uparrow$ & \textbf{SIM}$\uparrow$ & \textbf{NSS}$\uparrow$ \\
%            \midrule
            %\textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} 
 %               & 0.5763 & 0.0480 & 0.3059 & 0.1126 \\
%            \textbf{evST}~\cite{chane2024event}       
%                & 0.7848 & 0.2750 & 0.1396 & 1.4141 \\
%            \textbf{SEST (this work)}                  
%                & \textbf{0.7725} & \textbf{0.4725} & \textbf{0.4708} & 1.1434 \\
%            \bottomrule
%        \end{tabular}
%    }
%\end{table}


\subsubsection{Generalizability and Transferability on real event dataset}
We evaluated the cross-dataset generalizability of SEST in two complementary settings (Table~\ref{tab:generalizability_tab}). First, we assess synthetic-to-synthetic transfer by training on one synthetic dataset and testing on the other. The results show that training on N-DHF1K generalizes better to N-UCF Sports than the other way around. This suggests that DHF1K, which contains more diverse scenes and motion patterns, provides a richer training distribution that transfers more effectively to UCF Sports. Conversely, the more domain-specific sports content in UCF Sports leads to reduced generalization when evaluated on the broader DHF1K dataset.

Second, to assess generalization beyond synthetic data, we conduct a zero-shot evaluation on 100 sequences (sampled at 30Hz, equally distributed across the 6 scene categories) from the real event camera dataset of~\cite{chane2024event}, using 14 temporal bins and no fine-tuning. Despite the domain shift, SEST remains competitive: while evST obtains a higher NSS (1.4141), SEST achieves substantially higher CC and SIM (0.4725 and 0.4708), confirming generalizable saliency distributions. SNNevProto, in contrast, fails to generalise on AUC-J, CC, and NSS. SEST's lower NSS likely reflects its sensitivity to fixation-level spatial displacement under domain shift, and the low-motion nature of the real dataset may favosr evST's asynchronous per-pixel design. This highlights a limitation of the current real dataset and motivates N-DHF1K and N-UCF Sports as essential resources, given their broader motion dynamics, for training robust event-based saliency models.



\begin{table}[H]
    \centering
    \caption{Cross-dataset generalization. The top rows report synthetic-to-synthetic transfer between N-UCF Sports and N-DHF1K. The bottom rows report zero-shot evaluation on the real event camera dataset ~\cite{chane2024event} (no fine-tuning).}
    \label{tab:generalizability_tab}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt}
    \resizebox{0.6\textwidth}{!}{
        \begin{tabular}{llcccc}
            \toprule
            \textbf{Model (Train / Test)} & \textbf{\#bins} & \textbf{AUC-J} $\uparrow$ & \textbf{CC} $\uparrow$ & \textbf{SIM} $\uparrow$ & \textbf{NSS} $\uparrow$ \\
            \midrule
            \multicolumn{6}{l}{\textit{Synthetic-to-synthetic transfer}} \\
            \textbf{SEST (N-UCF Sports / N-DHF1K)} & 14 & 0.7831 & 0.2598 & 0.2246 & 1.2331 \\
            \textbf{SEST (N-DHF1K / N-UCF Sports)} & 14 & 0.9015 & 0.5286 & 0.4256 & 2.6873 \\
            \midrule
            \multicolumn{6}{l}{\textit{Zero-shot on real event data~\cite{chane2024event}}} \\
            \textbf{SNNevProto}~\cite{dangeloEventDrivenBioinspired2022} & 14 & 0.5763 & 0.0480 & 0.3059 & 0.1126 \\
            \textbf{evST}~\cite{chane2024event} & 14 & \textbf{0.7848} & 0.2750 & 0.1396 & \textbf{1.4141} \\
            \textbf{SEST (this work)} & 14 & 0.7725 & \textbf{0.4725} & \textbf{0.4708} & 1.1434 \\
            \bottomrule
        \end{tabular}
    }
\end{table}


\subsection{Computational Load}
We evaluated the inference time for a single saliency map prediction across all three models on both GPU and CPU (Table~\ref{tab:computational_tab}), using an NVIDIA RTX A5500 (16GB) and an Intel Core i9-12950HX. Despite its larger memory footprint, SEST achieves the fastest inference on both hardware configurations (6.62ms GPU, 121.68ms CPU). The high inference times of competing methods reflect their differing design goals: SNNevProto was optimized for the SpiNNaker neuromorphic platform~\cite{furber2020spinnaker}, where it achieves 16ms ~\cite{dangeloEventDrivenBioinspired2022}, while evST was designed for per-pixel saliency updates at microsecond precision rather than dense map reconstruction~\cite{chane2024event}, making direct latency comparison with frame-based approaches inherently limited. Table~\ref{tab:computational_tab} should therefore be read as a characterization of SEST's computational profile on general-purpose hardware, not as a ranking of overall efficiency.

%\begin{table}[hbt!]
%    \centering
%    \renewcommand{\arraystretch}{1.2}
%    \setlength{\tabcolsep}{6pt}
%    \resizebox{0.48\textwidth}{!}{
%        \begin{tabular}{llcccc}
%            \toprule
%            \textbf{Model} & \textbf{# bins} & \textbf{ GPU Inference time (ms)}  & \textbf{ CPU Inference time (ms)}  & \textbf{Model Size (MB)}\\
%            \midrule
%            \textbf{D'Angelo } & 14 & 877.7 & \textbf{19546.5} & - \\ 
%            \textbf{Simon Chane} & 14 & - & \textbf{2109.68} & - \\
%            \textbf{Ours} & 14 & 92.7 & 1703.6s & 180.247 \\
%
%            \bottomrule     
%        \end{tabular}
% }
%    \caption{Computational load(Results yet to be updated)}
%    \label{tab:computational_tab}
%\end{table}



\begin{table}[H]
    \centering
    \caption{Comparative inference times.}
    \label{tab:computational_tab}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt}
    \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{llcccc}
            \toprule
            \textbf{Model}  & \textbf{ GPU Inference time (ms)}  & \textbf{ CPU Inference time (ms)}  & \textbf{Parameters (M)} & \textbf{Model size (MB)}\\
            \midrule
            \textbf{SNNevProto \cite{dangeloEventDrivenBioinspired2022}} &  62.69 & 1396.17 & -  & - \\ 
            \textbf{evST \cite{chane2024event}} & - & 2109.68 & -  & - \\
            \textbf{SEST (this work)} &  \textbf{6.62} & \textbf{121.68} & 45.1 & 180.247 \\
            \bottomrule    
        \end{tabular}
 }
\end{table}

\subsection{Ablation study}
In this section, we assess the impact of two design choices on the N-UCF Sports test set: the learnable center bias component and the use of 2D convolutions in place of 3D convolutions within the decoder.

\subsubsection{Training without center bias learning} To evaluate the contribution of the spatial prior, we conducted an ablation study by training the architecture without the learnable center-bias component across all temporal configurations. The comparative results are detailed in Table \ref{tab:no_center_bias}. Our analysis indicates that the effectiveness of the center-bias is highly dependent on the temporal window length. At moderate temporal windows (10-14 bins), the center-bias significantly improves the CC and NSS metrics. We attribute this improvement to the module’s implementation as a multiplicative spatial gain, $\hat{Y} \odot (1 + \mathbf{M}_b)$, which allows the network to adaptively amplify salient features within statistically probable regions of interest.

However, at 21 bins, the effectiveness  diminishes.  We interpret this as a conflict between the learned global spatial prior and the increased local variance of longer sequences; as the temporal window expands, the salient target is more likely to deviate from the statistically learned center-bias regions, leading to a suppression of valid features. These results suggest the center-bias is most effective for short-to-medium temporal integration.

\subsubsection{Replacing Conv3d with Conv2d}: We also trained a variant of the model in which all 3D convolutions in the decoder are replaced by 2D convolutions, deferring the recovery of the temporal axis to the very last layer. When trained on 14 bins, this variant yields degraded performance (AUC-J: 0.8483, CC: 0.4072, SIM: 0.2415, NSS: 1.9544), as expected, since Conv2d treats each time bin independently and cannot exploit temporal correlations until the output. Reducing the input to a single bin provides only a marginal improvement (AUC-J: 0.8410, CC: 0.4179, SIM: 0.2946, NSS: 2.0522), still falling short of the Conv3d baseline. These results indicate that 2D convolutions are not well suited to the task given our pretrained backbone and underline the importance of explicitly modeling the temporal information of event-based data, a property that future work should further exploit to improve performance.

\begin{table}[H]
    \centering
    \caption{SEST performance on N-UCF Sports without center bias learning.}
    \label{tab:no_center_bias}
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6pt}
    \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{llcccc}
            \toprule
            \textbf{Model} & \textbf{\#bins} & \textbf{AUC-J} $\uparrow$ & \textbf{CC} $\uparrow$ & \textbf{SIM} $\uparrow$ & \textbf{NSS} $\uparrow$ \\
            \midrule
            SEST (No Center bias) & 21 & 0.8954 & 0.5190 & 0.3498 &  2.6149\\
            SEST (No Center bias) & 14 & 0.8847 & 0.4978 & 0.3795 &  2.5049\\
            SEST (No Center bias) & 10 & 0.8861 & 0.4799 & 0.3516 &  2.4906\\
            SEST (No Center bias) & 7 & 0.8999 & 0.4908 & 0.3595 &  2.4978 \\
            \bottomrule     
        \end{tabular}
 }
\end{table}
%\textbf{Predicting static saliency maps}:

%\begin{table}[hbt!]
%    \centering
%    \renewcommand{\arraystretch}{1.2}
%    \setlength{\tabcolsep}{6pt}
%    \resizebox{0.48\textwidth}{!}{
%        \begin{tabular}{llcccc}
%            \toprule
%            \textbf{Model} & \textbf{# bins} & \textbf{AUC-J} $\uparrow$ & \textbf{CC} $\uparrow$ & \textbf{SIM} $\uparrow$ & \textbf{NSS} $\uparrow$ \\
%            \midrule
%            \textbf{D'Angelo } & 1 & \textbf{0.936} & \textbf{0.707} & \textbf{0.565} & 3.863 \\ 
%            \textbf{Simon Chane} & 1 & \textbf{0.936} & 0.705 & 0.560 & \textbf{3.908} \\
%            \textbf{Ours (Conv2D)} & 1 & 0.926 & 0.671 & 0.534 & 3.523 \\

%            \bottomrule     
%        \end{tabular}
% }
%    \caption{Static saliency maps tab on DHF1K (Results yet to be updated)}
%    \label{tab:static_tab}
%\end{table}


%\subsubsection{Generalizability of our model} We also evaluated the cross-dataset generalizability of SEST (Table \ref{tab:generalizability_tab}). In the first setting, the model is trained on the N-UCF Sports dataset and tested on the N-DHF1K dataset. In the second setting, we do the opposite. The results show that training on the N-DHF1K dataset generalizes better to N-UCF Sports than the other way around. This suggests that DHF1K, which contains more diverse scenes and motion patterns, provides a richer training distribution that transfers more effectively to UCF Sports. On the other hand, the more domain-specific sports content in the UCF Sports dataset leads to reduced generalization when evaluated on the broader DHF1K dataset. 

%\begin{table}[hbt!]
%    \centering
%    \caption{Cross-dataset generalization.}
%    \label{tab:generalizability_tab}
%    \renewcommand{\arraystretch}{1.2}
%    \setlength{\tabcolsep}{6pt}
%    \resizebox{0.48\textwidth}{!}{
%        \begin{tabular}{llcccc}
%            \toprule
%            \textbf{Model (Train/test)} & \textbf{\#bins} & \textbf{AUC-J} $\uparrow$ & \textbf{CC} $\uparrow$ & \textbf{SIM} $\uparrow$ & \textbf{NSS} $\uparrow$ \\
%            \midrule
%            \textbf{SEST (N-UCF Sports / N-DHF1K)} & 14 & 0.7831 & 0.2598 & 0.2246 & 1.2331 \\
%            \textbf{SEST (N-DHF1K / N-UCF Sports)} & 14 & 0.9015 & 0.5286 & 0.4256 & 2.6873 \\
%            \bottomrule 
%        \end{tabular}
% }
    
%\end{table}


% ROMARIC : Check if true?
%Additional component-level ablations, such as variations of window sizes or decoder depth, were found to yield marginal differences relative to overall performance trends and were therefore omitted for clarity.
%
%Our results consistently demonstrate that the proposed design choices, rather than increased model capacity alone, are responsible for the observed improvements.

